Distant Representatives for Rectangles in the Plane

The input to the distant representatives problem is a set of $n$ objects in the plane and the goal is to find a representative point from each object while maximizing the distance between the closest pair of points. When the objects are axis-aligned rectangles, we give polynomial time constant-factor approximation algorithms for the $L_1$, $L_2$, and $L_\infty$ distance measures. We also prove lower bounds on the approximation factors that can be achieved in polynomial time (unless P = NP).

==> approx-continued-fraction.tex <==
%\subsection{A general approximation algorithm for all norms}

\subsection{Optimization problem for $L_1$ and $L_2$}
\label{sec:L-1,2-optimization-alg}

In this section we give an approximation algorithm for the optimization version of distant representatives for rectangles in the $L_1$ and $L_2$ norms. 
Define a \emph{critical} value to be a right endpoint of an interval where {\sc Placement} succeeds.  See Figure~\ref{fig:critical}. 


We use the following results whose proofs can be found below.
% Therese: reinserted this, since it was not clear to me when reading the paper

\begin{lemma}
\label{lem:closed=on-right}
{\sc Placement} succeeds at critical values, i.e., the intervals where {\sc Placement} succeeds are closed at the right.  Furthermore, a critical value provides an $f_\ell$-approximation.
%The intervals of values $\delta$ where {\sc Placement} succeeds are closed at the right.  
%\anna{We artificially engineered this with the tricky definition of big rectangles.}
\end{lemma}

\begin{figure}[htb]
    \centering
    \includegraphics[width=.58\textwidth]{Figures/critical-values.pdf}
    \caption{An illustration of critical values.}
    \label{fig:critical}
\end{figure}

%\begin{observation}
%A critical value provides an $f_\ell$-approximation.    
%\end{observation}

Thus our problem reduces to finding a critical value.

\begin{lemma}
\label{lemma:detect-critical}
The {\sc Placement} algorithm can be modified to detect critical values.
%\anna{We need this for Approach 1 described below.  I suspect we need it for Approach 2 as well.  
\end{lemma}

\begin{lemma}
\label{lemma:critical-bits-bound}
In $L_1$ any critical value $\delta$  is a rational number with numerator and denominator at most $4Dn$.  In $L_2$ for any critical value $\delta$, $\delta^2$ is a rational number with numerator and denominator at most $8D^2n^2$. 
%the number of bits in the numerator and denominator are bounded by a polynomial in $\log D$ and $\log n$. 
\end{lemma}
%\anna{Graeme proves this below.  I will verify it independently and put a proof here.}

%\attention{Now we have two possible approaches.}
%\anna{Well, Cabello's is a third possible approach: use binary search to narrow down to a small interval, then generate all critical values in that interval and binary search them.}

Based on these lemmas, we use continued fractions to find a critical value.
We need the following properties of continued fractions.
%\anna{needs a reference.}
\begin{enumerate}
\item A continued fraction has the form $a_0 + \frac{1}{a_1 + \frac{1}{a_2 + \cdots \frac{1}{a_k}}}$, where the $a_i$'s are natural numbers.

\item Every positive rational number $\frac{a}{b}$ has a continued fraction representation. Furthermore, %if $a$ and $b$ are bounded by $G$ then 
the number of terms, $k$, is $O(\log (\max\{a,b\}))$.  This follows from the fact that computing the continued fraction representation of $\frac{a}{b}$ exactly parallels the Euclidean algorithm; see~\cite[Theorem 4.5.2]{Bach-Shallit} or the wikipedia page on the Euclidean algorithm~\cite{wiki_euclididean}.
% https://en.wikipedia.org/wiki/Euclidean_algorithm#Continued_fractions
For the same reason, 
each $a_i$ is bounded by $\max\{a,b\}$.


\item Suppose we don't know $\frac{a}{b}$ explicitly, but we know some bound $G$ such that $a,b \le G$, 
and we have a test of whether a partial continued fraction is 
greater than, less than, or equal to $\frac{a}{b}$.  Then we can find the continued fraction representation of $\frac{a}{b}$ as follows. For $i=1 \ldots \log G$, use binary search on $[2..G]$ to find the best value for $a_i$.  
Note that the continued fraction with $i$ terms is increasing in $a_i$ for even $i$ and decreasing for odd $i$, and we adjust the binary search correspondingly.
In each step, we have a lower bound and an upper bound on $\frac{a}{b}$ and the step shrinks the interval.
If the test runs in time $T$, then
the time to find the continued fraction for $\frac{a}{b}$ is $O(T (\log G)^2)$, plus the cost of doing arithmetic on continued fractions (with no $T$ factor).
%\anna{Note: if we use doubling search instead of binary search, plus some more results on the Euclidean algorithm, we can get down to a single $\log$ factor.}
\end{enumerate}

\subparagraph*{Algorithm for $L_1, L_2$.}
Run the continued fraction algorithm using {\sc Placement} (enhanced to detect a critical value) as the test. The only difference from the above description is that we do not have a specific target $\frac{a}{b}$; rather, our interval contains at least one critical value and we search until we find one.  At any point we have two values $b_l$ and $b_u$ both represented as continued fractions, where {\sc Placement} succeeds at $b_l$ and fails at $b_u$, so there is at least one critical value between them.
We can use the initial interval $[1/n, 2D]$.  
To justify this, note that if 
{\sc Placement}($\frac{1}{n}$) fails , then $f_\ell/n > \delta^*$ by Theorem \ref{thm:placement}, so we get an 
$f_\ell$-approximation by using the representative points for $\delta = \frac{1}{n}$
(see the remark after Claim~\ref{claim:delta-bounds}). 
%\therese{try to improve this?}
%\anna{Ok, it's awkward to refer to the proof of the claim, but putting this tidbit into the claim proof does not seem better.}


%\graeme{Moved this paragraph up} \anna{I think this is worth saying, but it should go later since it's more of a detail and we should describe the main idea first.} \graeme{I agree. I'll leave it here for now, we can discuss it on Thursday.}

%\anna{The next two paragraphs give upper and lower bounds on $\delta^*$ which may still be relevant for the continued fraction approach.}

\remove{ this is Graeme's proof of Claim~\ref{claim:delta-bounds}
%
First, note that no solution exists with points distance $2D$ apart, so may as well assume $\delta < 2D$. Second, if there are two identical 0 by 0 rectangles, then $\delta^* = 0$. We can determine if this is the case in $O(n\log n)$ time. If this is not the case, then we note that because the instance has integer coordinates, then $\delta^*  \ge \frac{1}{n-1}$. \graeme{Is this obvious? Is the proof that follows needed?} This is a fairly trivial lower bound: place a grid of points $\frac{1}{n-1}$ distance apart. All rectangles with non-zero dimensions will intersect at least $n$ points, and 0 by 0 rectangles will hit one point. 0 by 0 rectangles can be matched to the sole grid point that overlaps the rectangle. The remaining rectangles can be matched trivially. As a result, one may as well only run {\sc Placement} with $\delta \in (\frac{1}{n}, 2D)$.
}

For the runtime, we use the bound $O(T(\log G)^2)$ from point 3 above, plugging in $T = O(n^2 \log n)$ for {\sc Placement} and the bounds on $G$ from Lemma~\ref{lemma:critical-bits-bound}, to obtain a runtime of $O(n^2 {\rm polylog}(nD))$, 
which proves Theorem~\ref{theorem:opt-alg} for $L_1$ and $L_2$.

The run-time for Theorem~\ref{theorem:opt-alg} can actually be improved to $O(n^2(\log n)^2)$ (i.e., without the dependence on $\log D$) with an approach that is very specific to the problem at hand (and similar to Cabello's approach).  
%Namely, we can generate a set $O(n^2)$ values within a small range and guarantee that at least one is critical.  We then sort this set and perform the binary search to find a critical values.  
The details are complicated for such a relatively small improvement and hence omitted here.


%\therese{We now have three files that start with approx-cabello and store bits and pieces of the details.  Could someone clean them out a bit, i.e., figure out whether we need all three, and perhaps add a short commentary at the beginning of each how they are different?}

%\graeme{They actually contain old stuff. I've moved them into old folder.}

%\anna{Discuss the run time of the algorithm.  Using the bounds from Lemma~\ref{lemma:critical-bits-bound} together with point 3 above and the $O(n^3)$ bound on {\sc Placement}, we get  $O(n^3 (\log D + \log n)^2)$.  } 

\remove{
\noindent
{\bf APPROACH 2.  Binary search followed by continued fractions}.  Described in more detail by Graeme below.
Do binary search (with calls to {\sc Placement}) until the interval $[s,t]$ is so small it only contains one rational number within our bounded number of bits (from Lemma~\ref{lemma:critical-bits-bound})---which must then be our desired critical value.  Then use continued fractions (without calling {\sc Placement}) to find the critical value. 

\noindent{\bf Pros and Cons}
Approach 2 might have a faster runtime because we call {\sc Placement} $O(\log D)$ times in the initial binary search and don't call it at all in the continued fraction search.  However, the dominant term in our run time is $O(n^3)$ so I don't think we should fuss about $\log$ or $\log^2$.

For Approach 2, we are relying on the precise number of bits in the critical values.  We MUST have only one critical value when we stop the binary search.  Then we would take the continued fraction representations for $s$ and $t$, take the common prefix of the two representations, and search for the next term, say the $i$th term.  I feel leery of this. Why should the $i$th terms for $s$ and $t$ only differ by 1? And if they differ by more, are all those options in the interval $[s,t]$?    

\attention{The end of the summary of the two approaches.}
} % end remove

\subparagraph*{Missing proofs.}  For space reasons we can here only give the briefest sketch of the proofs of Lemmas~\ref{lem:closed=on-right}, \ref{lemma:detect-critical}, and~\ref{lemma:critical-bits-bound}; details are in %Appendix~\ref{app:proofs}. 
the full version.
A crucial ingredient is to study what must have happened if {\sc Placement}($\delta$) goes from success to failure (when viewing its outcome as a function that changes over time $\delta$).

%\anna{I'd like to switch notation to 
%$\delta_1$ and $\delta_2$ (older comments are in the .tex}
%\attention{The awkward thing is that we're using subscripts for the different norms!  Yikes.  I will leave $\delta$ and $\delta'$.}

%We complete this section by giving the proofs of Lemmas~\ref{lem:closed=on-right}, \ref{lemma:detect-critical}, and~\ref{lemma:critical-bits-bound}.
%We view the outcome of {\sc Placement}($\delta$) as a function that changes over time $\delta$.
%We need the following:

\begin{observation}
\label{obs:events}
Assume {\sc Placement}($\delta$) succeeds but {\sc Placement}($\delta'$) fails for some $\delta'>\delta$.  Then at least one of the following
events occurs 
%between 
as we go from $\delta$ to $\delta'$:
%\anna{``between'' is not directional}
\begin{enumerate}
\item the set of small/big rectangles changes,
\item the distance between the centres of two small rectangles equals $\hat{\delta}$ for some $\delta\leq \hat{\delta}<\delta'$,
\item the set of blocker-shapes owned by a small rectangle increases,
\item the set of blocker-shapes intersecting a big rectangle decreases.
\end{enumerate}
\end{observation}

Roughly speaking,  Lemma~\ref{lem:closed=on-right} 
can now be  shown by arguing that such events do not happen in a sufficiently small time-interval before {\sc Placement} fails (hence the intervals where it fails are open on the left).  Lemma~\ref{lemma:critical-bits-bound} holds because there necessarily must have been an event at time $\delta$, and we can analyze the coordinates when events happen.  
Finally Lemma~\ref{lemma:detect-critical}  is achieved by running {\sc Placement} at time $\delta$ and also symbolically at time $\delta+\varepsilon$. 


==> approx.tex <==
\section{Approximating the   optimization problem}
\label{sec:optimization-alg}

%\anna{This section needs to be polished.  Start with statements of the best results (rather than starting with a basic result and then refining it). 
%Plan (with Graeme): eliminate Theorem 13, 14.  Keep Theorem 15 ($L_\infty$) and Section 4.2 (for L1 and L2). https://www.overleaf.com/project/5eb2b5a16347b50001a0f454 Eliminate the last section.}
%\graeme{I have done this. I backed up what was in this section before (see approx-old.tex). Simply modify main.tex to revert. }

In this section we 
use %the approximate decision algorithm 
{\sc Placement} to 
design approximation algorithms for the optimization version of the distant representatives problem for rectangles:

\begin{theorem}
\label{theorem:opt-alg}
There is an $f_\ell$-approximation algorithm for the distant representatives problem on rectangles in the $L_\ell$-norm, $\ell=1,2,\infty$ with run time $O(n^2 (\log n)^2)$ for $L_\infty$ and run time $O(n^2 {\rm \ polylog} (nD))$ for $L_1$ and $L_2$. 
Here (as before) $f_1 = 5, f_2 = \sqrt{34} \approx 5.83, f_\infty = 6$.
\end{theorem}


One complicating factor is that {\sc Placement} is not monotone, i.e., it may happen that {\sc Placement} fails for a value $\delta$ but succeeds for a larger value $\delta'$. %\anna{For example (just for us, probably too long for ESA), suppose we have a horizontal segment $R$ that just touches the bottom point of a  $+$-shape at $R$'s right endpoint.  Then $R$ is classed as big.  But if $\delta$ increases slightly, $R$ becomes small so we use its centre as $p(R)$ and this can kill a nearby other blocker-shape that was the only match for rectangle $R'$.  }
%\therese{I don't find the reference to Fig. 4 helpful; all it illustrates is what not-monotone means.  Could we add to/modify Figure 1 such that with a slightly smaller $\delta$ two big rectangles compete for one blocker-shape and so {\sc Placement} would fail?}
%\changed{The situation is illustrated in  Figure~\ref{fig:critical}.}
%\anna{The figure is just helpful for Section 3.2, so we could refer to it only there.}
We note that Cabello's algorithm~\cite{cabello2007approximation} behaves the same way.
%
We deal with $L_\infty$ in 
Section~\ref{sec:L-infty-optimization-alg} and with $L_1$ and $L_2$ in Section~\ref{sec:L-1,2-optimization-alg}.
\remove{
For $L_\infty$ we show that $\delta_\infty^*$ takes on one of $O(n^3)$ possible values, and then use binary search to find a good approximation.
%to $\delta_\infty^*$.   
%
For the other two norms,  
we do not know a
nice bound on the number of potential values of $\delta^*$ and we instead resort to searching the values of $\delta$ where {\sc Placement} changes its behaviour.  
We first show that the intervals of values $\delta$ where {\sc Placement} succeeds are closed at the right (this depends on our tricky definition of big rectangles).  We call these right endpoints \emph{critical} values of $\delta$. 
It is easy to observe that a critical value of $\delta$ provides 
%a good 
an $f_\ell$-approximation.
We show that {\sc Placement} can be used to detect critical values.
%, i.e., if Placement($\delta$) fails then Placement($\delta - \epsilon$) also fails for small enough $\epsilon>0$.
Next we show that if $\delta$ is a critical value for $L_1$ then $\delta$ is a rational with bounded bit complexity, and if $\delta$ is a critical value for $L_2$ then $\delta^2$ is a rational with bounded bit complexity. 
Finally, we show how to search for critical values using continued fractions. 
}
%\therese{Removed outlook here since the sections are now so short.}

We need some upper and lower bounds on $\delta^*$.  Note that if the input contains two rectangles that are single identical points, then
$\delta^*=0$.  Since this is easily detected, we assume from now on that no two input rectangles are single identical points.
%We need the following bounds on $\delta^*$.

\begin{claim}
\label{claim:delta-bounds}
%If two rectangles are single identical points then $\delta^* =0$. Otherwise 
We have $1/n \le \delta^* \le 2D$. 
\end{claim}
\begin{proof}
%The claims are obvious except the lower bound of  $1/n$.  
The upper bound is obvious.  For the lower bound, place
a grid of points %$\frac{1}{n-1}$  %Anna: this is correct, but maybe easier to digest if we just use n
distance $\frac{1}{n}$ 
 apart. All rectangles with non-zero dimensions will intersect at least 
$n+1$
%$n$ 
points, and 
single-point
%0 by 0  %Therese: I find "0 by 0" ugly.  If you really want it, then replace everywhere
rectangles will hit one point.  
Since no two single-point rectangles are identical, they
%Any 0 by 0 rectangle 
can be matched to the sole grid point that overlaps the rectangle. The remaining rectangles can be matched trivially. 
%Initially assign the centre of each rectangle as its representative point, and then (for all rectangles that are not single points) move the representative of the $i$th rectangle by exactly $i/n$ horizontally or vertically within the rectangle to obtain a set of representatives with distance at least $1/n$. % or more.
\end{proof}
%We can furthermore assume {\sc Placement}($\frac{1}{n}$) succeeds, if not, then $f_\ell/n > \delta^*$ by Theorem \ref{thm:placement}, so the solution of points distance $\frac{1}{n}$ apart is already the $f_\ell$-approximation we are looking for. 
Note that a solution with distance at least $\tfrac{1}{n}$ can be found easily, following the steps above.
% TB: To make it more tolerable that we refer to this later.


\subsection{Optimization problem for $L_\infty$}
\label{sec:L-infty-optimization-alg}

%In this section we give an approximation algorithm for the optimization version of Distant Representatives for rectangles in 
% Therese: I'm all for warm-ups, but it feels that we had *just* said this.
For the $L_\infty$ norm we use the following result about the possible optimum values; a proof is in
the full version. 
%Appendix~\ref{app:candidates}.

\begin{lemma}
\label{lemma:n-cubed}
In $L_\infty$, $\delta^*_\infty$ takes on one of the  $O(n^3)$ values of the form $(t-b)/k$ where $k \in \{1,\dots,n\}$ and $t,b$ are rectangle coordinates. 
%More precisely, either $t$ is the top coordinate $t(R)$ of some rectangle  $R$ and $b$ is the bottom coordinate $b(R')$ of a different rectangle $R'$, or $t$ is the right $r(R)$ coordinate of some rectangle $R$ and $b$ is the left coordinate $\ell(R')$ of a different rectangle $R'$.
\end{lemma}

%\input{appendix_candidates.tex}

\newcommand{\calD}{\ensuremath{\mathcal{D}}}

%\anna{clean up the lemma and the part below to be consistent} 
%
%For the $L_\infty$-norm, we can make the number of iterations of binary search independent of $D$.

%The proof is below, but we first describe the algorithm.

%\attention{Option 1}

%{\bf Optimization algorithm for $L_\infty$.}
%{\bf Algorithm for $L_\infty$.}
Let $\Delta$ be the set of $O(n^3)$ values from the lemma.
%
%There is a set $\calD$ of $O(n^3)$ values such that
%$\delta_\infty^*\in \calD$,  
%see Lemma~\ref{lem:delta_form} (proved below \graeme{above now I believe}).  
%Furthermore, 
We can compute the set $\Delta$ in $O(n^3)$ time and 
sort it in $O(n^3 \log n)$ time.  
Say $\Delta = \{d_1,d_2,\dots,d_N\}$ in sorted order, and
set $c_i:=d_i/f_\infty$. 
Because of non-monotonicity, we cannot efficiently find the maximum $c_i$ for which {\sc Placement} succeeds.  
Instead, we use binary search to find $i$ such that {\sc Placement}($c_i$) succeeds but {\sc Placement}($c_{i+1}$) fails.
Therefore
%Then we claim that the representative points found by {\sc Placement}($c_i$) provide an $f_\infty$-approximation
%of the optimum assignment:
%since {\sc Placement}($c_{i+1}$) fails,  
$\delta^*_\infty < f_{\infty}c_{i+1} =  d_{i+1}$ which implies that  $\delta^*_\infty \le d_{i} = f_{\infty}c_i$ 
and the representative points found by {\sc Placement}($c_i$) provide an $f_\infty$-approximation.
%of the optimum assignment:


To initialize the binary search, we first run {\sc Placement}$(c_N)$, and, if it succeeds, return its computed representative points
 since they provide an $f_\infty$-approximation
of the optimum assignment. 
Also note that {\sc Placement}$(c_1)$ must succeed---if it fails then 
$\delta_\infty^*<f_\infty c_1=d_1$,
which contradicts $\delta_\infty^*\in \Delta$.
Thus we begin with the interval $[1,N]$ and perform binary search on within this interval to find a value $i$ such that {\sc Placement}($c_i$) succeeds but {\sc Placement}($c_{i+1}$) fails.


\remove{
% I rearranged to make it more top-down
We know that {\sc Placement}($c_1$) must
find an assignment, because otherwise $\delta_\infty^*<f_\infty c_1=d_1$,
which contradicts $\delta_\infty^*\in \calD$. We first verify whether {\sc Placement}($c_N$) fails, otherwise $c_N = d_N/f_{\infty} \ge \delta^*/f_{\infty},$ and so {\sc Placement}($c_N$) gives an $f_\infty$-approximation and we return this solution.
Otherwise perform binary search on $c_1,\dots,c_N$ to find $i$ where
{\sc Placement}($c_i$) returns an assignment while {\sc Placement}($c_{i+1}$) 
fails.  Therefore, since {\sc Placement}($c_{i+1}$) fails,  $\delta^*_\infty < f_{\infty}c_{i+1} =  d_{i+1} \implies \delta^*_\infty \le d_{i} = f_{\infty}c_i$. Therefore 
the assignment returned by {\sc Placement}($c_i$) is an $f_\infty$-approximation
of the optimum assignment.
} % end remove

%\changed{This algorithm takes time $O(n^3 \log n)$ for the sort, plus $O(n^2 \log n)$ for the $O(\log n)$ calls to {\sc Placement}.  We can improve this using a matrix searching technique of Frederickson and Johnson as described by Agarwal and Sharir~\cite[Section 3.3]{agarwal1998efficient}.
%The important feature of the values in $\Delta$ is that there are $O(n^2)$ numerators and $O(n)$ denominators.  We can sort the numerators in time $O(n^2 \log n)$ (whether this can be done faster is the famous $X+Y$ sorting problem).  We then have an $O(n^2) \times n$ matrix with sorted rows and columns, and the matrix search technique can be used.  We still use $O(\log n)$ calls to {\sc Placement}.   
%\anna I'm pretty sure that non-monotonicity does not mess this up
%The total run time becomes $O(n^2 \log n)$.
%This proves Theorem~\ref{theorem:opt-alg} for $L_\infty$.  
%Note that the number of calls to Placement is independent of $D$---unlike for $L_1$ and $L_2$, as we will see in the next subsection.
%} % end changed

%The important feature of the values in $\Delta$ is that there are $O(n^2)$ numerators and $O(n)$ denominators. 
We can get away with sorting just the $O(n^2)$ numerators and performing an implicit binary search, to avoid the cost of generating and sorting all of $\Delta$. Let $t$ be the sorted array of $O(n^2)$ numerators, which takes $O(n^2\log n)$ time to generate and sort. The denominators are just $[n]$, so there is no need to generate and sort it explicitly. Define the implicit \emph{sorted} matrix $a$, where $a[r, c] = t[r] / (n-c)$, for $0\le r\le |t|-1, 0 \le c \le n-1$. Each entry of $a$ can be computed in $O(1)$ time. Since the matrix is sorted, the matrix selection algorithm of Frederickson and Johnson \cite{frederickson1984generalized} can be used to get an element of $\Delta$ at the requested index in $O(n \log n)$ time. Using selection, one can perform the binary search on $\Delta$ implicitly. While accessing elements of $\Delta$ takes more time, it is still less than the time to call {\sc Placement} on the element accessed. Each iteration of the binary search is dominated by the runtime of {\sc Placement}, so the total runtime is 
$O(n^2(\log n)^2)$. 
This proves Theorem~\ref{theorem:opt-alg} for $L_\infty$. 

%}
\remove {% Therese: I guess we've decided not to use this?
\attention{even newer}

\therese{Two major changes:  (1) Cleanup in the beginning, don't give the full $O(n^3\log n)$ algo first.  (2)  Explicitly say how to do the search,
rather than appealing to FredericksonJohnson.  It gets a bit simpler that way because we don't really need to cut at the true median, as long
as we cut a fraction off. } 

%{\bf Optimization algorithm for $L_\infty$.}
\subparagraph*{Algorithm for $L_\infty$.}
Let $\Delta$ be the set of $O(n^3)$ values from the lemma.
%We can compute the set $\Delta$ in $O(n^3)$ time and 
%sort it in $O(n^3 \log n)$ time.  
Say $\Delta = \{d_1,d_2,\dots,d_N\}$ in sorted order, and
set $c_i:=d_i/f_\infty$.
(We will not actually compute or sort $\Delta$, but assume here that we have it for ease of explanation.)
Because of non-monotonicity, we cannot efficiently find the maximum $c_i$ for which {\sc Placement} succeeds.
Instead, we use a recursive search to find $i$ such that {\sc Placement}($c_i$) succeeds but {\sc Placement}($c_{i+1}$) fails.
Therefore
%Then we claim that the representative points found by {\sc Placement}($c_i$) provide an $f_\infty$-approximation
%of the optimum assignment:
%since {\sc Placement}($c_{i+1}$) fails,  
$\delta^*_\infty < f_{\infty}c_{i+1} =  d_{i+1}$ which implies that  $\delta^*_\infty \le d_{i} = f_{\infty}c_i$
and the representative points found by {\sc Placement}($c_i$) provide an $f_\infty$-approximation.
%of the optimum assignment:

We could easily find this $i$ in $O(n^3\log n)$ time by doing binary search after computing and sorting $\Delta$, but
give here a faster approach which is similar to the matrix selection algorithm of Frederickson and Johnson
\cite{frederickson1984generalized}.
To initialize, compute the set $E$ of $O(n^2)$ possible numerators \anna{changed ``enumerators'' to ``numerators''.  I guess we don't want $N$ instead of $E$ though.}
in $\Delta$; for each $e\in E$ we
will also store an interval $D(e)$ of possible denominators (initially $D(e)=\{1,\dots,n\}$ for all $e$).
We can compute $d_1=\min_{e\in E} \tfrac{e}{n}$ and $d_N=\max_{e\in E} e$ along the way.
Run {\sc Placement}$(d_N/f_\infty)$, and, if it succeeds, return its computed representative points since they provide an $f_\infty$-approximation
of the optimum assignment.   So from now on we assume that {\sc Placement}($d_N/f_\infty$) fails.
Note that {\sc Placement}($d_1/f_\infty$) must succeed since otherwise $\delta_\infty^*<d_1$, which contradicts
$\delta_\infty^*\in \Delta$.
So we may from now on assume that we have $d_s,d_f$ (initially $d_1$ and $d_N$) such that $d_s<d_f$,
{\sc Placement}($d_s/f_\infty$) succeeds and {\sc Placement}($d_f/f_\infty$) fails.     We also
maintain that $d_s$ and $d_f$ are the minimum/maximum among all {\em candidates}, i.e., all values $\tfrac{e}{k}$ with $e\in E$ and $k\in D(e)$.

To find $i$, first compute $\sum_{e\in E} |D(e)|$, which takes $O(n^2)$ time since the size of interval $D(e)$ can
be computed in constant time.
This is the number of candidates that are left, including $d_s$ and $d_f$.  If this has constant size then we can find $i$
with brute force in $O(n^2)$ time by calling {\sc Placement} on all of them.
Otherwise, we eliminate at least a quarter of the candidates as follows.
First compute the set $\mathcal{M}=\{\tfrac{e}{m(e)}: e\in E\}$, where $m(e)$ is the median of $D(e)$.  This
takes $O(n^2)$ time since $m(e)$ can be found in constant time from the interval.   Then find the weighted median in $\mathcal{M}$, where $\tfrac{e}{m(e)}$
has weight $|D(e)|$; this can be done in $O(|\mathcal{M}|)=O(n^2)$ time.    We call this weighted median $d_j$ though we do not compute its index $j$ in $\Delta$.
Run {\sc Placement}$(d_j/f_\infty)$, and if it succeeds, replace $d_s$ by $d_j$; otherwise replace $d_f$ by $d_j$.
Finally (and crucially) update some of the intervals $D(e)$.  Say {\sc Placement}($d_j/f_\infty$) succeeded (the other case is symmetric).
For each $e\in E$, we can eliminate any index $k\geq e/d_j$ from $D(e)$ since the corresponding candidate satisfies $\tfrac{e}{k}\leq d_j$.  (One exception: We keep one copy of $d_j$.)  Because $d_j$ was the weighted median of $\mathcal{M}$, and each element $\tfrac{e}{m(e)}$ in $\mathcal{M}$ was the median of the candidates at $e$, we eliminate at least a quarter of the candidates (and likely more).    Also $d_j$ is the minimum item of the remaining candidates as required.

So the number of candidates is a fraction smaller with each recursion, and each recursion takes $O(n^2+{\sc Placement})$ time, leading to $O((n^2+{\sc Placement}\log n)$ run-time in total.  
}

%\anna{We should keep in mind that we can reduce to $O(n^2 \log n)$ to sort the numerators (using the matrix search technique of Frederickson and Johnson) plus $O(\log n)$ calls to Placement.  This is relevant in case we can reduce the run-time of Placement below $n^3$.} 

%The total run-time is $O(n^3\log n)$ plus $O(\log n)$ executions of
%{\sc Placement}($c_i$).  In total, this is $O(n^3 \log n)$ so we
%have proved Theorem~\ref{theorem:opt-alg} for $L_\infty$.  
%Note that the number of calls to Placement is independent of $D$---unlike for $L_1$ and $L_2$, as we will see in the next subsection.

%\begin{theorem}
%There exists a  $6$-approximation algorithm for
%the distant representative problem in the $L_\infty$-norm
%with run-time $O(n^3 \log n)$.
%\end{theorem} 


\remove{
\medskip
It remains to prove Lemma~\ref{lemma:n-cubed}.

\anna{This part (below) can be simpler.  I suggest: assume $x$ and $y$ ordering known.  Note (maybe via LP constraints): $x$ and $y$ are independent, i.e. we can shift $x$ coordinates (keeping $y$ fixed) so long as any distance $\ge \delta^*$ stays $\ge \delta^*$.  If no $x$ at left boundary, shift them all leftward.  If no $x$ at right boundary, then argue how to shift each successive one by $\epsilon / n$ times index.
This will be like below, but separated into $x$ and $y$, and each of those is really the 1D argument.}

In this section we show that for the $L_\infty$-norm there exists a {\em finite} set $S$ (of size $O(n^3)$) 
of possible values for $\delta_\ell^*$.
%\anna{well, a poly. bound also implies a finite set.}  
Moreover, set $S$ can be described using only the coordinates of the input rectangles.

We call a rectangle $R_j$ {\em left represented in $P$} if $x_j=\ell_j$,
i.e., its representative is at its left side, and similarly for the
other three directions.
We call a rectangle $R_j$ {\em left-constrained in $P$} if there
exists some other rectangle $R_i$ such that $x_j=x_i+\delta$.
In other words, the representative of $R_i$ prevents the representative of $R_j$ from being
further left.
Similarly define {\em bottom-constrained} with respect to $y$-coordinates.


\begin{lemma}
\label{lem:tight}
In the $L_\infty$ norm,
there exists an optimal solution such that all rectangles
are left-constrained or left-represented, and bottom-constrained
or bottom-represented.
\end{lemma}
\begin{proof}
We only give the argument for ``left'', the other argument is symmetric.
Among all solutions with
optimal distance $\delta^*$, take one that minimizes the
sum of the coordinates of the assigned representatives.

Assume that some rectangle $R_j$ is neither left-constrained
or left-represented in this solution.
Then $\varepsilon= \min\{x_j - \ell_j,
x_j - \max_{i: x_i+\delta^*\leq x_j} \left(x_i + \delta^*\right)\}$)
is positive.    Use $x_j':=x_j-\varepsilon$ as new coordinate of
the point that represents $R_j$.  By choice of $\varepsilon$ this
point still lies within $R_j$, and has horizontal distance at least
$\delta^*$ from all other points.  Since vertical distances have not
changed and we are in the $L_\infty$-distance, therefore the new set
of representatives is again feasible, but its sum of coordinate is
smaller, a contradiction.
\end{proof}

We call a solution that satisfies the conditions of Lemma~\ref{lem:tight} a {\em tight} solution.

\begin{corollary}
\label{cor:tight}
For any tight optimal solution, any $x$-coordinate $x_j$ has the
form $\ell_h+k\, \delta^*$ for some left boundary-coordinate $\ell_h$
and some integer $k\in \{0,\dots,n-1\}$.

Likewise any $y$-coordinate $y_j$ has the form
form $b_{h'}+k'\, \delta^*$ for some bottom boundary-coordinate $b_{h'}$
and some integer $k'\in \{0,\dots,n-1\}$.
\end{corollary}
\begin{proof}
We only show the first claim, the other is symmetric.
Sort the
representatives by increasing $x$-coordinates and prove the claim for $x_i$
by induction on $i$.    Rectangle $R_1$ is left-represented, because
there is no representative with smaller $x$-coordinate and so it cannot
be left-constrained.  Therefore $x_1=\ell_1$.  For $j>1$, rectangle
$R_j$ is either left-represented (then $x_j=\ell_j$) or left-constrained.
If the latter, then $x_j=x_i+\delta^*$ for some $x_i<x_j$, which means
$i<j$.  We know by induction that $x_i=\ell_h+k\cdot \delta^*$ for some
index $h$ and integer $k<i$.  Therefore $x_j=\ell_h+(k+1)\delta^*$.
\end{proof}


\begin{lemma}
\label{lem:delta_form}
For the $L_\infty$-norm,
the optimal $\delta^*$ has one of the following two forms:
\begin{itemize}
\item $(r_j-\ell_i)/k$ for some indices $i\neq j$ with $\ell_i<r_j$ and
        some integer $k\in \{1,\dots,n-1\}$, or
\item $(t_j-b_i)/k$ for some indices $i\neq j$ with $b_i<t_j$ and
        some integer $k\in \{1,\dots,n-1\}$.
\end{itemize}
\end{lemma}
\begin{proof}
Take a tight optimal solution.
We have two good cases:
\begin{enumerate}
\item Some rectangle $R_j$ is right-represented and left-constrained.
       Then         $\delta^*=(r_j-\ell_h)/k$ as desired.
\item Some rectangle $R_j$ is top-represented and bottom-constrained.
        Likewise then $\delta^*$ is of the desired form.
\end{enumerate}

The claim is that one of these cases must apply.  Assume for
contradiction that neither of them applies; we will show that then
$\delta^*$ was not maximal.  To this end, define
$\varepsilon$ to be the minimum of the following values:
\begin{itemize}
\item $\varepsilon_1 = \frac{1}{n} \min\{r_j-x_j: \text{$R_j$ is not right-represented}\}$. 

\item $\varepsilon_2 = \frac{1}{n} \min\{t_j-y_j: \text{$R_j$ is not top-represented}\}$.
\item $\varepsilon_3 = \frac{1}{n} \min_{j: \text{$R_j$ is not left-constrained}} \{x_j - \max_{i: x_i+\delta^*\leq x_j}\{x_i + \delta^*\} \, \}$.
\item $\varepsilon_4 = \frac{1}{n} \min_{j: \text{$R_j$ is not bottom-constrained}} \{y_j - \max_{i: y_i+\delta^*\leq y_j}\{y_i + \delta^*\} \, \}$.
%       \text{$R_j$ is not left-constrained} \}$.
\end{itemize}
        $\varepsilon_1,\varepsilon_2$ are positive by definition of
        right-represented and top-represented, and
        $\varepsilon_3,\varepsilon_4$ are positive by definition of left-constrained and bottom-constrained.
        So $\varepsilon=\min \{
        \varepsilon_1,\dots ,\varepsilon_4\} > 0$.
        Define a new set of representatives $P'$ where point $(x_i',y_i')$ for $R_i$ is chosen as follows:
        \begin{itemize}
        \item Set $x'_i$ to be $x_i$ if $R_i$ was right-represented in $P^*$.
        \item Otherwise, $\varepsilon_1$ was chosen such that $x_i + n\varepsilon \leq x_i + n\varepsilon_1\leq r_i$.
        Set $x_i'=x_i+ \sigma_x^{-1}(i) \cdot  \varepsilon \leq r_i$, where
        $\sigma_x^{-1}(i)\leq n$ is the index that $x_i$ would get if we sorted by $x$, i.e.,
        $x_{\sigma_x(1)} \leq x_{\sigma_x(2)} \leq \dots \leq x_{\sigma_x(n)}$.


    \item Set $y'_i$ to be $y_i$ if $R_i$ was top-represented in $P^*$.
    \item Otherwise, $\varepsilon_2$ was chosen such that $y_i + n\varepsilon \leq y_i + n\varepsilon_1\leq r_i$.
                Set $y_i'=y_i+ \sigma_y^{-1}(i) \cdot  \varepsilon \leq r_i$, where
                $\sigma_y^{-1}(i)\leq n$ is the index that $y_i$ would get if we sorted by $y$.
    \end{itemize}

        We claim that for any $i<j$ the representatives of $R_i$ and $R_j$
        in $P'$ have distance at least $\delta'=\delta^*+\frac{1}{n}\varepsilon$.
        To see this, recall that $p_i$ and $p_j$ were sufficiently separated
        in at least one dimension; up to renaming and symmetry we may hence
        assume $x_j\geq x_i+\delta^*$.  Since $\delta^*$ is positive, therefore
        $\sigma_x^{-1}(i) < \sigma_x^{-1}$  which implies $\sigma_x^{-1}(i) \leq \sigma_x^{-1}(j)-1$.

                If $R_j$ is not right-represented, then $x_j'=x_j+ \sigma_x^{-1}(j) \cdot \varepsilon$
                while $x_i'\leq x_i+\sigma_x^{-1}(i) \cdot \varepsilon \leq x_i + \sigma_x^{-1}(j)\cdot \varepsilon - \varepsilon$.
                So $x_j'-x_i'\geq x_j-x_i + \varepsilon \geq \delta^*+\varepsilon$ and they are separated by at least $\delta'$.


                So assume that $R_j$ is right-represented.
                Since Case 1 does not apply, $R_j$ was not left-constrained.
                By choice of
                $\varepsilon_3$ we have $x_i+ \delta^*+\varepsilon \leq x_i + \delta^* + \varepsilon_3 \leq x_j$, so $x_i+\delta'
                \leq x_j$ and they are sufficiently separated.
\end{proof}
}

%%%%%%%%%%%%%%%%%%%%


%To develop an approximation algorithm from the decision problem, 
%We first sketch a simple idea to give an \graeme{NOPE}$f_\ell+\varepsilon$ approximation.  Let us use {\sc Placement}($\delta$) for the algorithm implicit in Theorem~\ref{thm:placement}, i.e., the algorithm either
%finds an assignment of representatives of distance at least $\delta$, or 
%reports that $\delta_\ell^* < f_\ell \delta$, where $f_\ell$ is a constant that
%depends only on the used norm $L_\ell$.

%To turn {\sc Placement} into an approximation algorithm, the simplest approach is to
%do (roughly speaking) a binary search for $\delta_\ell^*$.     
%Observe that $0\le \delta_\ell^*\leq 2D$ (where $D$ is an upper bound on coordinates). {\sc Placement}(0) succeeds and {\sc Placement}($2D$) fails.
%We perform binary search in $[0,2D]$ until the remaining interval has size 
%$\varepsilon$.  If {\sc Placement} succeeds with the midpoint of the interval, we set the lower bound to the midpoint, otherwise we set the upper bound to the midpoint. Thus
%we reach some value $t$ such that
%{\sc Placement}($t$) returns an assignment while {\sc Placement}($t{+}\varepsilon$) returns
%that $\delta_\ell^*< f_\ell(t{+}\varepsilon)$.  
%The run-time for this is $O(\log D+\log(\tfrac{1}{\varepsilon}))$ executions 
%of {\sc Placement}($\delta$). 
%Note that $\log D$ is polynomial in the input-size since this many bits
%are required to describe the input-coordinates.    
%So as long as we choose $\varepsilon$ suitably, e.g. $\varepsilon = 1/n$,
%the algorithm runs in polynomial time. The points given by {\sc Placement}($t$) gives and $f_\ell + $\graeme{This is what Theorem 13 used to say, %but is now much shorter. Will delete or }




\input{approx-continued-fraction}

% Independent in log(D). More detail if we wanted.
%\input{approx-cabello-short}

